Prompting Audios Using Acoustic Properties For Emotion Representation

Emotions lie on a continuum, but current models treat emotions as a finite valued discrete variable. This representation does not capture the diversity in the expression of emotion. To better represent emotions we propose the use of natural language descriptions (or prompts). In this work, we address the challenge of automatically generating these prompts and training a model to better learn emotion representations from audio and prompt pairs. We use acoustic properties that are correlated to emotion like pitch, intensity, speech rate, and articulation rate to automatically generate prompts i.e. 'acoustic prompts'. We use a contrastive learning objective to map speech to their respective acoustic prompts. We evaluate our model on Emotion Audio Retrieval and Speech Emotion Recognition. Our results show that the acoustic prompts significantly improve the model's performance in EAR, in various Precision@K metrics. In SER, we observe a 3.8% relative accuracy improvement on the Ravdess dataset.

==> latexfiles/analysis.tex <==
\subsection{Analysis}
To analyze the impact of the linguistic and acoustic variability of synthesized speech on WER, we analyze how the WER decreases with respect to the increase in the vocabulary size of the training data.
Figure \ref{fig:vocab_wer} shows the training vocabulary size and the WER on test-other subset in two experiments, i.e. $\mathrm{L+A}$ and $\mathrm{A}$. As a reminder the training data in $\mathrm{L+A}$, speech from new text is being synthesized whereas in experiment $\mathrm{A}$, speech from repetitive text is added.
We can observe that there is a negative correlation between the training vocab size and the WER. For test-other and test-clean, the Pearson correlation between WER and training vocab size is $-0.8$, and $-0.9$ respectively.
This observation is similar to that reported in \cite{gody2023unsupervised}, where new topic words were introduced in the training vocabulary and an improvement in WER was observed. 
\begin{figure}
    \centering
    \includesvg[width=0.6\linewidth,height=0.6\linewidth]{figures/vocab_wer.svg}
    \caption{Training vocab size and the WER on test other in two experiments, i.e. $\mathrm{L+A}$ and $\mathrm{A}$, as a function of training hours of synthetic data used in ASR.}
    \label{fig:vocab_wer}
\end{figure}

We also evaluate the silence, graphemes, and word duration for the different experiments. Figure \ref{fig:boxplot} shows the box plot of silence durations in the synthesized speech used in experiments $\mathrm{L+A}$, $\mathrm{L}$, compared to the real speech. (These silences do not include the beginning and end silences). We observe that the silence duration in the $\mathrm{L+A}$ experiment is higher on average than the ones in $\mathrm{A}$ experiment and the real data.
This is also observed for the grapheme durations. It has been reported previously that slower speech rates actually lead to better ASR performance \cite{meng2022don}, which is what we observe in these experiments as well. 

Figure ~\ref{fig:qqplot} shows the qq-plot for the average word duration for the experiment $\mathrm{L+A}$ compared with $\mathrm{A}$, $\mathrm{L+A}$ compared with the real data, and the experiment $\mathrm{A}$ compared with real data. It can be observed that the data used in experiment $\mathrm{L+A}$, has durations most similar to the ones of the real data (lies closer to the 45 degree line). This also explains why the experiment $\mathrm{L+A}$ has better performance than the experiment $\mathrm{A}$. 

 \begin{figure}
    \centering
    \includesvg[width=0.4\linewidth,height=0.4\linewidth]{figures/boxplot_silences.svg}
    \includesvg[width=0.4\linewidth,height=0.4\linewidth]{figures/boxplot_grapheme.svg}
    \caption{Box plot comparing distribution of silences and graphemes in the two synthesized dataset and the real data.}
    \label{fig:boxplot}
\end{figure}

\begin{figure}
    \centering
    \includesvg[width=0.3\linewidth,height=0.3\linewidth]{figures/qqplot_LA_A.svg}
    \includesvg[width=0.3\linewidth,height=0.3\linewidth]{figures/qqplot_A_Real.svg}
    \includesvg[width=0.3\linewidth,height=0.3\linewidth]{figures/qqplot_LA_Real.svg}
    \caption{qq-plot for the average word duration for two sets of synthesized data with compared with each other and the real data. Left-to-right: $\mathrm{L+A}$ vs. $\mathrm{A}$, $\mathrm{L+A}$ vs. real, $\mathrm{A}$ vs. real.}
    \label{fig:qqplot}
\end{figure}

==> latexfiles/experiments.tex <==
% \vspace{-0.05cm}
% \subsection{Evaluation Setup}
% We evaluate the model for and under various settings. \\

% \noindent \textbf{Prompt Analysis}: 
% \vspace{-0.1in}
\subsection{Prompt Analysis}
% \vspace{-0.05in}
To evaluate which of the proposed acoustic prompts are better [and to see if any of them are better than the class label]. We apply the trained model on emotion classification in a supervised classification setting. The model is trained 6 different times, where each time the description associated with the emotion audios are different. Among the 6, 1 is using the class label alone, 4 are using the acoustic prompts as described in Section 4, and 1 is using the prompt augmentation - combines all the acoustic prompts. 

% \vspace{-0.15in}
\subsection{Emotion Classification}
[Why are we doing this experiment]
How using these prompts could help in emotion classification. We have one zero-shot like setup (where we leave one dataset out for testing). Then then we pre-trained model from previous setup and finetune it on the left-out dataset. 

% \subsection{Out of Domain Classification}
% \vspace{-0.1in}
\subsubsection{Leave one out}
% \vspace{-0.1in}
[Why are we doing this exp]
1. How well the model generalizes to a new dataset. We want to see how a model trained on predefined set of classes generalizes to the same or different classes in a new dataset. 
[Define mismatch][distributional shift]
To perform mismatch emotion classification, out of the 6 emotion datasets, we leave one out for testing and train the model on the other 5 emotion datasets. In case where Ravdess is the testing dataset, `calm' class is not represented in any of the other 5 emotion datasets and could be considered zero shot classification result. 
In case of Crema-d, all the emotion classes are represented in the training classes. 
% There may or may not be an overlap of the emotion classes between the training and testing datasets. For example, when testing on Ravdess, 

% \vspace{-0.15in}
\subsubsection{Finetune}
% \vspace{-0.1in}
[Why are we doing this exp]
We want to see how using the acoustic prompts at pretraining stage would benefit the classification. 
% \vspace{-0.05in}
We perform supervised classification on the testing subsets of 2 emotion datasets. Once the model is trained on 5 emotion datasets leaving one specific dataset out. The model then acts as a feature extractor and an additional 3 fully connected layers are trained on top using the training folds of the left out dataset. 
% ELABORATE ON THE PARAMETERS

% \vspace{-0.15in}
\subsection{Emotion Audio Retrieval}
% \vspace{-0.1in}
In order to access whether the trained model learns the associations between the acoustic prompts and the respective acoustic properties, we perform audio retrieval on the emotion datasets. We make queries similarly to the prompts as described in Section 4. An example of query is `high male pitch anger'.
For a given query, the model outputs top $K$ audios whose audio embeddings have highest cosine similarity to the text embedding of the query. For the top $K$ audios, since we know the true acoustic prompts, we can evaluate how good the model's outputs is w.r.t the query. 
% ## Retrieval results 

==> latexfiles/result_discussion.tex <==
% \vspace{-0.1cm}
\begin{table*}[tbh!]
\caption{Accuracy achieved when the model is trained under different settings and tested on the left out dataset (shown in the  col 2,3) and when finetuned on the dataset (shown in the col 4,5). 4D refers to the 4 audio captioning datasets used in original CLAP model. ED refer to Emotion Datasets.}
    \centering
    \begin{tabular}{lcc|cc}
         \toprule
         & \multicolumn{2}{c}{Leave one out dataset} & \multicolumn{2}{c}{Finetune}  \\
         \toprule
         Training dataset & Crema-d & Ravdess & Crema-d & Ravdess \\
         \midrule
         Random & 16.67 & 12.50 & & \\
         4D & 17.85 &	15.99 &	67.29	& 68.50 \\
        5 ED - \textit{class label} & 	35.22&	22.88 & x & x \\
        4D + [5 ED - \textit{class label}] &	34.68 &	38.46  &	72.86&	68.69\\
        4D + [5 ED - \textit{prompt augmentation}] &	33.00 &	27.88 &	72.56	& 72.46\\
        SoTA & & & 75.20 & 80.21 \\
        \bottomrule
        \vspace{-1cm}
    \end{tabular}
    \label{tab:ood_supervised_results}
\end{table*}


% \vspace{-0.1in}
\subsection{Prompt Analysis}
% \vspace{-0.05in}
\begin{figure}[tbh!]
  \centering
  \vspace{-0.3cm}
%   \includegraphics[width=0.7\linewidth,height=0.3\linewidth]{images/prompt_cremad}
%   \includegraphics[width=0.45\linewidth,height=0.4\linewidth]{images/prompt_ravdess}
  \includesvg[width=0.45\linewidth,height=0.6\linewidth]{images/prompt_cremad}
  \includesvg[width=0.45\linewidth,height=0.6\linewidth]{images/prompt_ravdess}
  \caption{Accuracy achieved using different prompts on CREMA-D (left) and RAVDESS (right). A=class-label, B=pitch-prompt, C=intensity-prompt, D=speech-rate-prompt, E=articulation-rate-prompt, F=prompt-augmentation.}
    \label{fig:prompt_analysis}
          \vspace{-0.1in}
\end{figure}
For prompt analysis, we train the model on 4 audio captioning datasets and 1 emotion dataset. Figure \ref{fig:prompt_analysis} shows the performance achieved when the model is trained on the training set and tested on the testing sets of Ravdess and Crema-d respectively.
We observe that among the 4 acoustic prompts, pitch prompt gives the best performance. Next best performance is achieved by the intensity prompt. This can be observed in both Ravdess and Crema-d. On Crema-d, articulation rate prompt performs better than speech rate prompt but the reverse is observed in Ravdess. [WHY]   
Secondly, we observe that overall prompt augmentation is giving the best performance in both datasets. This is encouraging to see due and it validates the original hypothesis that using acoustic prompts would help the emotion classification. 
% ADD ABOUT THE CLASS RPOMPT
% \vspace{-0.3cm}
\subsection{Emotion Classification}
% \vspace{-0.1in}
\subsubsection{Leave one out}
% \vspace{-0.05in}
% ## ood results 
We perform 4 experiments, shown in columns 2,3 of Table~\ref{tab:ood_supervised_results}. Firstly, we train the model on only 4 audio captioning datasets (4D) and evaluate on Ravdess and Crema-d. This is zero shot classification since none of the emotion classes are represented in the training datasets. We achieve 17.85\% accuracy on Crema-d and 15.99\% on Ravdess. 
Secondly we train on only 5 ED, leaving one dataset out. When trained on all 5, excluding Crema-d, we achieve 35.22\% on Crema-d. When trained on all 5 ED except for Ravdess and tested on it, we achieve 22.88\%.  
Thirdly we train the model on all 4D and 5ED, leaving one out. We achieve 34.68\% on Crema-d, which is a slight degradation from the second experiment.
Done similarly on Ravdess, we see a lot of improvement, boosting performance to 38.46\%.
Lastly, this experiment setting is similar to the third one except that for the ED, we perform prompt augmentation. We observe that it slightly degrades performance on both datasets. For Crema-d the performance drops to 33\% and for Ravdess to 27.88\%. 

There are two learnings from these results. Firstly adding ED is helping the performance on a new emotion dataset. Secondly, prompt augmentation's results are similar to the results obtained when trained using only the class label. This is in contrast to what was observed in Section 6.1, and we hypothesize that this is because of the amount of data. When the training data size is large, like in the current experiment, the benefit from using the acoustic prompts decrease. 

[In 6.1, we do not have mismatch condition, but there there is a mismatch condition. The mismatch condition is quite strong and results in this drop in performance. ]
[However we do observe improvement when we include dataset in the training in next section. ]

% \vspace{-0.2in}
\subsubsection{Finetune}
% \vspace{-0.05in}
[Takeway] 
Fine tuning show that adding prompt augmentation kinda of improves performance. In ravdess, we improved performance by absolute 4\%. In crema-d the performance did not improve, but the accuracy is about the same as when the prompt augmentation is not used. 

The results for supervised classification are shown in columns 4,5 of Table~\ref{tab:ood_supervised_results}. 
Firstly when the model is trained on only 4D and finetuned on Crema-d, we achieve 67.29\%, when done similarly for Ravdess we achieve 68.5\%.
Secondly when trained on 4D and 5ED and finetuned on the chosen datasets, we observe performance improvement in both the datasets; 72.8\% in Crema-d and 68.69\% in Ravdess.
Thirdly when we train a model on 4D and 5ED including prompt augmentation, we observe a slight decrease in performance for Crema-d. The performance improves for Ravdess to 72.46\%. [WHY]
We perform 5 fold cross validation for both datasets. Note that we dont perform the experiment where the model is only trained on only 5ED due to our observation in section 6.2.1 where 4D+5ED lead to better performance than 5ED alone. 

% \begin{table}[]
%     \caption{Accuracy achieved when the model is trained under different settings and tested on the left out dataset.}
%     \centering
%     \begin{tabular}{lcc}
%     \toprule
%         &  \multicolumn{2}{c}{Leave one dataset out} \\
%         % \hline
%         Training Dataset & Crema-d & RAVDESS  \\
%         \midrule
%         Random & 16.67 & 12.50 \\
%         4D & 17.85 &	15.99 \\
%         5 ED {class label} & 	35.22&	22.88\\
%         4D + [5 ED {class label}] &	34.68 &	38.46\\
%         4D + [5 ED + prompt augmentation] &	33.00 &	27.88\\
%          \bottomrule
%     \end{tabular}
%     \label{tab:zero_shot_results}
% \end{table}
% % ## Supervised classification result 
% \begin{table}[]
%     \caption{Accuracy achieved when the model is trained under different settings and then finetuned with on a specific training folds of the dataset.}
%     \centering
%     \begin{tabular}{lcc}
%     \toprule
%     %     &  \multicolumn{2}{c}{Dataset} \\
%     %     % \hline
%         Training Dataset & Crema-d & RAVDESS  \\
%     \midrule
%         SoTA & 75.20 & 80.21 \\
%         4D  &	67.29	& 68.50 \\
% 4D + [5 ED {class label}] &	72.86&	68.69\\
% 4D + [5 ED + 5 prompt augmentation]  &	72.56	& 72.46 \\ 
% \bottomrule
%     \end{tabular}
%     \label{tab:supervised_results}
% \end{table}



% \vspace{-0.35in}
% \vspace{-0.7cm}
\subsection{Audio Retrieval}
% \vspace{-0.05in}
[Where do we use audio retrieval.][We want to know if the acoustic property are connected and this retrieval allows to evaluate the emotions in the continuum] [How the retrieval numbers compare to audio retrieval precision numbers. cite the paper]
Figure~\ref{fig:retrieval} shows the results of audio retrieval. We calculate precision@$K$ for each acoustic prompt shown on the x-axis. 
% Precision@$K$ is the proportion of relevant items that come up in top $K$ items. 
[Takeaway at the top here]. [This suggests that we can introduce more elaborate descriptions, and be to retrieve audios including the descriptions.]
We evaluate using 3 different models, one trained on 4D, one trained with an additional 5 ED, and the third with an additional of prompt augmentation. We observe that the model trained on all datasets, and using prompt augmentation performs the best in all cases. The takeaway here is that our model is able to retrieve audio significantly better when trained using prompt augmentation. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth,height=0.5\linewidth]{images/retrieval.png}
    \caption{Precision@K achieved when the trained model under different settings is used for the audio retrieval task.}
    \label{fig:retrieval}
\end{figure}

==> latexfiles/results.tex <==
\subsection{Synthetic speech vs Real speech}
Figure \ref{fig:hm_synthetic} shows the WER decrement when more data is subsequently added to the ASR training. For the test-other subset in Librispeech, it can be observed that with 100 hours of synthetic data, we can beat the performance of 10 hours of real data. To reach the performance of 50 hours of real data, we need about 500 hours of synthetic data and for 100 hours of real data, 1K hours of synthetic data is needed. Therefore about 10 times more synthetic data than real data is needed to achieve similar ASR performance.

For the test-clean part of Librispeech, the performance on 100 hours of synthetic speech approximately matches the performance of 10 hours of real speech, 400 hours of synthetic speech beats 50 hours of real speech and 600 hours of synthetic speech beats 100 hours of real speech. For the cleaner audios in test-clean, about 7 times more synthetic data than real data is required to achieve similar ASR performance. 

If we assume the presence of little paired data, i.e. 100 hours, then adding 960 hours of synthetic data, we can beat the performance of 100 hours of real data on test-other (this can be seen in the next section). This is encouraging to see that with little paired data, we can improve the performance by adding additional synthetic data. This reduces the real paired data required and therefore makes the ASR fine-tuning for a new domain a relatively cheaper process.

Note: Since the evaluation data is out of domain for the initial model and only fine-tuned for 20 epochs, the WER reported is much higher than the SoTA \cite{chung2021w2v, kim2023branchformer}.

\begin{figure}
    \centering
    \includesvg[width=0.45\linewidth,height=0.6\linewidth]{figures/hm_synthetic_test_other.svg}
    \includesvg[width=0.45\linewidth,height=0.6\linewidth]{figures/hm_synthetic_test_clean.svg}
    \caption{WER comparison when different hours of synthetic data is included into training. The horizontal lines indicate the WER when only 10, 50 and 100 hours of real data is used in training. Left chart and right chart show the results on test-other and test-clean respectively.}
    \label{fig:hm_synthetic}
\end{figure}

\subsection{Linguistic vs Acoustic variability in Synthetic Speech}

In the following experiments, we assume 100 hours of paired data from Librispeech train. In the first experiment, the remaining 860 hours of Librispeech train are synthesized and added into training. In the successive experiments, an additional 100 hours of unpaired text is selected and used for speech synthesis and included in the training data. We control for the lexical and acoustic variability incorporated in the training data by controlling for the source of the additional 100 hours of text/synthesized speech pairs. 

% Figure \ref{fig:L_A_comparison} compares the effect on the WER when subsequently adding synthetic data into training. In these experiments, we assume 100 hours paired data is available. In the first bar in the chart, in addition to 100 hours of paired data, we use the remaining 860 hours of Librispeech train and synthesize the text. 
% To add both linguistic and acoustic variability in the following experiments, we select 100 hours of data from another corpus, L-Text and synthesize it. In each following experiment, we select additional 100 hours from L-Text and add that to the training data and train the model again. 

To add only acoustic variability and no lexical (experiment denoted as `$\mathrm{A}$'), we select the additional 100 hours of data from Librispeech train again. This selected data is already present in the data in its synthesized form; another version of this synthesis is added to the training data again. The Voicebox model introduces variability in the speaker's gender, speaking style, speech rate, and therefore having two synthetic versions of the text, we introduce only acoustic variability into the data. 

To add only lexical variability and no acoustic (experiment denoted as `$\mathrm{L}$'), the additional 100 hours of data is selected from Libri-Text. We use the J-AT \cite{kim2022joint} strategy as explained before where the unpaired text is paired with averaged audio embeddings and used for model training. Since only new text is included and no audio is used, only lexical variability is incorporated into the model. 

To add both acoustic and lexical variability (experiment denoted as `$\mathrm{L+A}$'), similarly as above, the additional 100 hours of data is selected from Libri-Text. This selected data is synthesized and included in the training. Since the text and synthesized speech are new each time, both acoustic and lexical variability in introduced in the data. Figure \ref{fig:L_A_comparison} compares the three different settings. 

Firstly, it can be observed that with both linguistic and acoustic variability, the performance is better in both test-other and test-clean, as compared to when only acoustic or lexical variability is present individually. 
Furthermore, when more synthetic data is included in training the performance consistently improves for the $\mathrm{L+A}$ setting, slightly in the case of only acoustic variability and worsens in the case of lexical variability. And although, in the low-resource data settings, having lexical variability is better in both test-other and test-clean, with the increment in training data, having more acoustic variability turns out be better than only lexical variability (that is owing to the worsening performance of only lexical variability experiment).

Finally, it can be observed that it is better to use Voicebox model to synthesize the speech than use the unpaired text as-is. On average, using Voicebox leads to a $9.6\%$ relative WER improvement in test-other and a $8.0\%$ relative improvement in test-clean. At best, in the high-resource data experiments, the synthetic data setting leads to more improvement, namely $19.4\%$ in test-other and $19.8\%$ in test-clean.

\begin{figure}
    \centering
    \includesvg[width=0.7\linewidth,height=0.6\linewidth]{figures/L_A_test_other.svg}
    \includesvg[width=0.7\linewidth,height=0.6\linewidth]{figures/L_A_test_clean.svg}
    \caption{WER comparison when synthetic data is added into training. The green color bar shows the when the additional synthetic data is generated from new text - not already included in the training. The orange color bar shows when the additional synthetic data is generated from the text that the model has already seen, and the red color bar shows when the additional text is used as is, without any synthesis. Top and bottom chart show the results on test-other and test-clean respectively.}
    \label{fig:L_A_comparison}
\end{figure}

In the following section, we analyze the relationship between acoustic and lexical variability on WER. 

